Detecting Dispersed Radio Transients in Real Time Using Convolutional Neural Networks

We present a methodology for automated real-time analysis of a radio image data stream with the goal to find transient sources. Contrary to previous works, the transients we are interested in occur on a time-scale where dispersion starts to play a role, so we must search a higher-dimensional data space and yet work fast enough to keep up with the data stream in real time. The approach consists of five main steps: quality control, source detection, association, flux measurement, and physical parameter inference. We present parallelized methods based on convolutions and filters that can be accelerated on a GPU, allowing the pipeline to run in real-time. In the parameter inference step, we apply a convolutional neural network to dynamic spectra that were obtained from the preceding steps. It infers physical parameters, among which the dispersion measure of the transient candidate. Based on critical values of these parameters, an alert can be sent out and data will be saved for further investigation. Experimentally, the pipeline is applied to simulated data and images from AARTFAAC (Amsterdam Astron Radio Transients Facility And Analysis Centre), a transients facility based on the Low-Frequency Array (LOFAR). Results on simulated data show the efficacy of the pipeline, and from real data it discovered dispersed pulses. The current work targets transients on time scales that are longer than the fast transients of beam-formed search, but shorter than slow transients in which dispersion matters less. This fills a methodological gap that is relevant for the upcoming Square-Kilometer Array (SKA). Additionally, since real-time analysis can be performed, only data with promising detections can be saved to disk, providing a solution to the big-data problem that modern astronomy is dealing with.

==> notes.tex <==

\section{2021-01-03}
Extensively tested new sigma-clipping approaches.
\begin{enumerate}
    \item FFT Convolutions and global clipping
    \item FFT Convolutions and local clipping
    \item Patch-based with multiprocessing (fastest AIS, but least quality)
    \item 
\end{enumerate}

However, I did find that FFT convolution on PyTorch is very fast, even on CPUs.
That means I can return to my convolutional source-finder.

The quality control remains slow, on both PyTorch and NumPy, so I should leave it as an option.
Safe goes for sigma-clipping in general, a simple standard deviation should be sufficient.

==> sections/instrument.tex <==
\section{Instrument, Observations \& Simulations}
\label{sec:instrument}
\subsection{Instrument \& Observations}
Though intended to be generally applicable, the methods presented in this paper were designed using AARTFAAC.
AARTFAAC is a wide-field, fast cadence imaging, low-frequency radio facility designed to survey the Northern Hemisphere for bright low-frequency ($30-80\, \text{MHz}$) transient events.
It specialises in transients that evolve on timescales from one second to several minutes.
It can process data coming from LOFAR's low-band antennae (LBA) simultaneously with other LOFAR observations.
AARTFAAC uses 288 (576) dipoles and 6 (12) central LOFAR stations, resulting in a maximum baseline of $300 \text{m}$ (1.5\,km).
It obtains a spatial resolution of $1^\circ$ (20 arcmin) at 60MHz.
Sensitivity is best at Zenith, decreasing while approaching the horizon due to radio frequency interference and lower antenna sensitivity.
Correlation, calibration and imaging can already be done in streaming mode for AARTFAAC-6 \citep{prasad2016aartfaac}.
The brightest sources in the sky: Cygnus A, Cassiopeia A, Taurus A, Virgo A and the Sun are removed prior to imaging (in visibility space).
% Galactic emission is reduced by removing baselines shorter than $10 \lambda$ with $\lambda = 5 \text{m}$ at 60 MHz.
Finally, primary beam correction is applied, flattening the antenna response across the field of view \citep{kuiack2019aartfaac}.

For development of the methods in this study sixteen observing bands arranged in two sets of 8 consecutive subbands of 195.3 kHz calibrated bandwidth each, leading to two bands at 57.6MHz through 59.0 MHz and 61.1 MHz through 62.5 MHz, were used.
The integration time is 1 second.
Examples of AARTFAAC-6 images are given in \ref{fig:a6_clean}. 
% All 16 $1024 \times 1024$ pixel images generated are processed in parallel.
% Despite the fact that integrating over the subbands will yield higher SNR, keeping all of them has significant benefits for both spurious source rejection and actual transient detection and classification.
% Further elaboration will be given in Section \ref{sec:methodology}.



\subsection{Transient Simulation}
For our inference procedure (see Section \ref{sec:nn}) the most informative data product is the frequency-time intensity data, or dynamic spectrum, which is the final product of our data pipeline.
Using this array, we want to estimate (as fast as possible) physical parameters which help to classify the type of signal detected.
As specified earlier, to infer these parameters we will employ a neural network.
Since we have few true transient candidates, we are very short on data to train a neural network.
Favorably, we know one of the most important properties of a true astrophysical transient: a bright, broadband, dispersed signal. 
The dispersion of the signal is manifested through the broadening of the pulse over a finite bandwidth.
It originates from interaction of the emitted photons with electrons along the path between an observer and the source.
Thus, assuming a uniform density of free electrons, it gives an indication of the distance that a signal has traveled.
The integrated electron column density, called the dispersion measure (DM), is used as a proxy for the distance to the source.
Using known equations, we can easily simulate dispersed astrophysical transients.
The DM of non-astrophysical transients usually is close to 0 (i.e., no broadening of the pulse), making the DM possibly the most useful feature for separating signal from noise \citep{kuiack2020apparent}.
We build a dataset by injecting these simulated pulses into randomly sampled noise from the survey.
In the following, the reported values parameters and can be set according to the interests of the practitioner.
They should be set such that the simulated dataset covers the population of interest sufficiently.
First, we generate a Gaussian pulse profile using a width sampled uniformly between $0$ and $16$, corresponding to a maximum FWHM of $37.67$ seconds.
The profile is computed as 
\begin{equation}f(t, w) = \exp\left[-\left(\frac{t}{w}\right)^2\right]\end{equation} centered around $t_0$.
For each frequency $\nu$ of the survey, we compute the arrival time by applying a dispersion delay
\begin{equation}
t_\nu = t_0 + C_{\text{DM}} \text{DM}\left(\nu^{-2} - \nu_0^{-2} \right)
\end{equation}
with $C_{\text{DM}}$ the dispersion constant $ \frac{e^2 \text{pc}}{8 \pi^2 \epsilon_0 m_e c} \cdot 10^{-6}\approx 4148.806$  $\text{MHz}^2 \text{cm}^{-3} \text{ms}$ \citep{lorimer2012handbook}.
In this analysis, we sample the $\text{DM}$ uniformly between $0$ and $512$, covering a significant part of the known FRB population \citep{petroff2016frbcat}.
The final intensity is computed as
\begin{equation}
    I(\nu, t) = A\left(\frac{\nu}{\nu_0}\right)^\alpha f(t-t_\nu, \nu)
\end{equation}
where $A$ is the burst amplitude (arbitrary units), assuming a standard normal noise level.
We experimented with $A$ uniformly between $0$ and $32$ and $\alpha$, the spectral index, sampled from $(-4, 4)$ uniformly.
We compute the intensity for all time-steps and frequencies and save the pulse at the corresponding band and time indices.
Using this procedure, we create $32,768$ samples (input time-frequency plots and output parameters pairs) to train the network.
Let $\bm \epsilon \in M \times T$ be a spatially integrated AARTFAAC-6 noise sample of $T$ consecutive time-steps at a random spatial location at $M$ frequencies.
We sample $16,384$ of such, using a maximum of $256$ sample locations per individual sequence.
This gives us $2^{14} \cdot 2^{16} = 2^{30} = 1,073,741,824$ possible signal-noise combinations.
This number increases even more when one considers all the temporal indices $t_0$ that the transient signal can be centered around in the data-point.
In this paper, we run experiments with $T=64$ and we centered the inserted transients around $t_0 \sim U(0, 64)$.
This enhances (next to the chosen network architecture, see Section \ref{sec:nn}) temporal invariance of the neural network.
Examples are given in Figure \ref{fig:sim_examples}.
It is clear from the examples that AARTFAAC6 operates with two separated consecutive ranges of sub-bands\footnote{We tested which configuration (e.g., two separate ranges, one continuous range) of sub-bands resulted in the best parameter estimates (\autoref{sec:nn}) and actually found that a single range works better.}.

% \begin{figure*}
%     \centering
%     \includegraphics[width=0.7\textwidth]{images/dm_inference/dm_inference.png}
%     \caption{Examples of generated pulses injected into AARTFAAC6 noise (amplified with a sampled scaling factor). ``Target'' denotes the DM that the pulse was simulated with, ``Prediction'' shows the neural network output and uncertainty.}
%     \label{fig:sim_examples}
% \end{figure*}

\begin{figure*}
    \centering
    \includegraphics[width=\linewidth]{images/dm_inference/burst_examples.pdf}
    \caption{Examples of generated pulses injected into AARTFAAC6 noise. We denote the parameters that the pulse was simulated with, as well as the predictions that the neural network output.}
    
    \label{fig:sim_examples}
\end{figure*}



\subsection{Skymap Simulation}
To test the source-finder, we carry out experiments using simulated all-sky images.
This has the advantage that we control entirely the noise characteristics and SNR of the sources.
First, we generate a model that simulates large-scale inhomogeneities of the final image. 
E.g., our Galactic foreground noise and Cygnus A \& Cassiopeia A calibration remnants.
An example is given in \ref{sec:bg_images}.
Then, we add to this map standard, independent Gaussian noise.
Finally, we add point sources at log-normally sampled flux densities $s \sim \log\mathcal{N}\left(\mu, \sigma^2\right)$, resulting in a flux distribution that has most of the density centered at a certain SNR, but with significant outliers.
These outliers cause substantial side-lobes throughout the image, testing our source-finder's robustness.
Finally, we convolve this image with a circularly symmetric low-pass filter, whose impulse response is given by
\begin{equation}
    h[n_1, n_2] = \frac{\omega_c}{2\pi \sqrt{n_1^2 + n_2^2}}J_1(\omega_c \sqrt{n_1^2 + n_2^2})
\end{equation}
where $J_1$ is the Bessel function of the first kind and order and we have $h[0, 0] = \frac{\omega_c^2}{4\pi}$.
$\omega_c$ is a parameter that controls the size of the beam.
Single-channel and integrated examples are given in \ref{sec:bg_images}.

==> sections/methodology/quality_control.tex <==
\subsection{Quality Control}
As specified earlier, we consider all 16 images output by the imaging pipeline.
This is motivated triply.
First, the dispersed signal of astrophysical (extra-galactical) transients means that integrating them over frequency with incorrect adjustment for dispersion will wash out the signal.
For this reason, we perform source detection and analysis in all subbands simultaneously (for more details, see \autoref{sec:source_detection}).
Second, occasionally one of these can be highly corrupted after strong interference, causing the correlation \& imaging pipeline to shoot to extreme values.
Integrating these directly would cause the entire time-step to be lost, as this corrupted sub-band will dominate the statistics.
Third, we can use the availability of images at multiple sub-bands to detect and filter terrestrial and near-Earth RFI which appears undispersed.
We describe these last two cases in the following.

Take an image-cube $\b X_t \in \mathbb{R}^{C \times D \times D}$ at time-step $t$ consisting of $C$ images of size $D \times D$, each corresponding to an individual sub-band.
For AARTFAAC6, we have $C=16$ and $D=1024$.
If available, $\b X_t$ is loaded into GPU memory.
% Occasionally, one of these can be highly corrupted after strong interference causes the correlation \& imaging pipeline to shoot to extreme values.
If any of these individual sub-band images is extremely corrupted, we simply filter it out based on maximum absolute value: $\max \text{ abs}\,\left(\mathbf{x}_t\right) > e$, where $\b {x}_t$ is a single sub-band in $\b X_t$. 
% We set $\epsilon = 1\cdot 10^5 \cdot \sigma$.
Images that exceed the threshold are imputed with zeroes.
An example of such poor quality image is given in Figure \ref{fig:cor_example}.

Now, we deal with the RFI cases. 
Though less obvious than the previously dealt with corruptions, strong RFI needs to be filtered as the side-lobes throughout the image will cause many false positives downstream.
These occur rather frequently, but favorably have a narrow bandwidth and often occur in only one bandpass.
The filtering is done based on a mean-square distance threshold and normalizing using robust statistics.
The idea is that we can leverage the fact that we have images coming from $C$ central frequencies at the same time, assuming that the majority of these are uncorrupted.
We compute the median image by taking the pixel-wise median over the $N$ images.
We square the difference of each image with this median and calculate the image mean for all of these.
This gives us a list $\b s$ of $C$ distance scores.
Next, we calculate the median and median absolute deviation of this list and standardize the scores.
\begin{equation}
\b z = \frac{\b s - \text{median}\,(\b s)}{\text{MAD} \, (\b s)}
\end{equation}
where $\text{MAD}$ stands for Median Absolute Deviation \citep[e.g.][]{howell2005median}.
Since we use robust center and spread statistics, outliers are easily picked up on. 
Using $z_h=5$ we found empirically that this is a very accurate approach to filtering RFI-corrupted images.

On simulated data, we tested by modelling RFI as extremely bright single-band point sources (1 to 4 times the PSNR). 
We retrieved 87\% of the RFI corrupted images.
Note that this is relatively mild RFI, so the false negatives are no surprise. 
Also, as the concern might arise that a highly dispersed transient might only appear in one channel, risking it to be filtered out as RFI.
%\footnote{The robustness of the pipeline is displayed here: \url{https://youtu.be/grZX9dVxXzk}. Note the stability of the detected sources.}.
However, reassuringly we report zero false positives for these.

Images that exceed this threshold are imputed with zeroes.
Note that this is a standardized score, thus not sensitive to user-specified settings or the particular survey.
Examples of RFI detections that were one subband adjacent to the clean images presented in Figure \ref{fig:a6_clean} are given in Figure \ref{fig:examples_rfi}.


==> sections/methodology/source_detction_old.tex <==
\subsection{Source Detection}
% As specified earlier, we take inspiration from \cite{spreeuw2018pyse} and \cite{swinbank2015lofar}.
We analyse images at multiple bandpasses at the same time in parallel and optionally on GPUs.
This is done since astronomical transients are expected to be dispersed over these bandpasses, and integrating them out before searching would decrease their SNRs.
Accordingly, this work searches in all frequencies simultaneously.

\subsubsection{Peak Detection}
\cite{swinbank2015lofar} and \cite{spreeuw2018pyse} divide the image to be analysed into a grid. 
In every patch, sigma-clipping is performed and thus local statistics are used for the detection threshold.
Although paralellizable, this procedure is too cumbersome to perform in real-time.
Instead, we approximate local statistics using convolutions.
This can be done in parallel extremely efficiently on a GPU, even for the batch of $N$ images.
Let $\b M_t \in \mathbb{R}^{N\times D \times D}$ be the background noise for $\b X_t$.
In the following, we omit the subscript $t$ to avoid cluttering.
\begin{equation}
    m_{h, i,j} = \sum_{n_1 = -k}^k \sum_{n_2 = -k}^k G(n_1, n_2) x_{h, i + n_1, j + n_2}
\end{equation}
where 
\begin{equation}
G(n_1, n_2) = \frac1Z \exp [-\frac1{2 \sigma^2} (n_1^2 + n_2^2)]
\end{equation} with $Z = \sum_{n_1=-k}^k \sum_{n_2=-k}^k \exp[-\frac{1}{2\sigma^2}(n_1^2 + n_2^2)]$. 
The subscript denotes the 3-dimensional index.
$\sigma$, the spread of the Gaussian, is a parameter.
It should be wide enough such that no significant source-specific flux is detected, but narrow enough such that sufficiently local noise (e.g., galactic background noise) will be picked up.
A robust heuristic that can determine $\sigma$ is, given a model of the PSF of the survey, sweeping over a range of candidate $\sigma$ and selecting the one that increases the signal of the main beam compared to the side-lobes the most.
$k$ is a truncation parameter that controls the computational cost. 
It should be set in accordance to the requested $\sigma$.
Note that (circular) boxcar filters can be used likewise.
We did not find a significant change of performance based on the choice of kernel.
The resulting $\b M$ is an approximation of the local noise level for each subband.
Additionally, to reduce the influence of side-lobes we estimate a local variance using a convolution.
\begin{equation}
    s^2_{h, i, j} = \sum_{n_1 = -k}^k \sum_{n_2 = -k}^k G(n_1, n_2) (x - m)^2_{h, i + n_1, j + n_2}
\end{equation}

First, $\b M$ is subtracted from $\b X$ to obtain a `flat' noise-corrected image $\b Y = \b X - \b M$.
We now apply a global iterative sigma-clipping procedure to estimate the entire background directly.
Using a while condition and a specified threshold $\kappa$ we iteratively exclude all pixels with values above $\mu_i + \kappa \sigma_i$ where $\mu_i$ and $\sigma_i$ are global center and spread estimates of $y$ (within a user-specified radius) at iteration $i$.
Finally, we correct for side-lobes by dividing (pixel-wise) over the local standard deviation: $z_{hij} = \frac{y_{hij}}{s_{hij}}$.
The intuition is as follows. 
In the neighbourhood of bright sources, many side-lobes are expected as spurious astronomical sources.
By correcting for the local variability, we exclude many of these.
Applying this step risks not detecting peaks that are in a close neighbourhood of multiple bright sources.
However, it excludes many false positives in a natural manner.
Moreover, by applying sigma-clipping locally, PySE \citep{spreeuw2018pyse} also will not pick up on faint sources in a neighbourhood of bright ones.

We obtain final source `islands' by thresholding $z$ using a user-specified $\lambda$. 
Setting $\lambda = 0$ will return all by sigma-clipping detected sources.
Setting $\lambda$ higher will exclude sources based on the local standard deviations.
Therefore, $\kappa$ acts as a retrieval parameter; setting it to a low value will recover many candidates, and $\lambda$ subsequently filters the retrieved candidates based on the local variability, making $\lambda$ a precision parameter.

Again, since values in $z$ are standardized the entire procedure is agnostic to the survey specifics. Examples of the procedure of noise estimation and variability are shown in Section \ref{sec:bg_images}.

% Let $b \in \{0, 1\}^{N \times D \times D}$ be the boolean array resulting from the element-wise thresholding: $b_{hij} = \mathbb{I}(z_{hij} > \lambda)$.
% This boolean array consists of 'islands' that correspond to source detections.
\subsubsection{Peak Localization}
In order to obtain the peak locations and values, we apply a maximum filter to $\b Y$.
\begin{equation}
    \tilde{y}_{h, i, j} = \max\{y_{h, n, m}: n, m \in  \{ i - k, \dots, i + k \} \times \{ j - k, \dots,    j + k \}\}
\end{equation}
with $k=3$.
Then, we obtain the peak locations $\b P \in \{0, 1\}^{N \times D \times D}$ by the following boolean operations:
\begin{equation}
    p_{hij} = \mathbb{I}(y_{hij} = \tilde{y}_{hij} \land z_{hij} > \lambda)
\end{equation}
where $\mathbb{I}(\cdot)$ denotes the indicator function.
Intuitively, we only include pixels that are both the local maximum and above the detection threshold, giving us the exact location of the peaks.

This concludes the source detection \& localization pipeline.
The advantages of all the previous operations are two-fold. 
First, they are fully parallel and accelerated on GPUs.
In our tests, 16 images ($N = 16$) $1024 \times 1024$ can be processed on an NVIDIA TitanRTX in less than a \textbf{tenth of a second} (see Section \ref{sec:results}).
Second, they are agnostic to survey specifics and only use standardised approaches and values, which should generalise well to other data.

